TGL: A General Framework for Temporal GNN Training on Billion-Scale Graphs

Many real world graphs contain time domain information. Temporal Graph Neural Networks capture temporal information as well as structural and contextual information in the generated dynamic node embeddings. Researchers have shown that these embeddings achieve state-of-the-art performance in many different tasks. In this work, we propose TGL, a unified framework for large-scale offline Temporal Graph Neural Network training where users can compose various Temporal Graph Neural Networks with simple configuration files. TGL comprises five main components, a temporal sampler, a mailbox, a node memory module, a memory updater, and a message passing engine. We design a Temporal-CSR data structure and a parallel sampler to efficiently sample temporal neighbors to formtraining mini-batches. We propose a novel random chunk scheduling technique that mitigates the problem of obsolete node memory when training with a large batch size. To address the limitations of current TGNNs only being evaluated on small-scale datasets, we introduce two large-scale real-world datasets with 0.2 and 1.3 billion temporal edges. We evaluate the performance of TGL on four small-scale datasets with a single GPU and the two large datasets with multiple GPUs for both link prediction and node classification tasks. We compare TGL with the open-sourced code of five methods and show that TGL achieves similar or better accuracy with an average of 13x speedup. Our temporal parallel sampler achieves an average of 173x speedup on a multi-core CPU compared with the baselines. On a 4-GPU machine, TGL can train one epoch of more than one billion temporal edges within 1-10 hours. To the best of our knowledge, this is the first work that proposes a general framework for large-scale Temporal Graph Neural Networks training on multiple GPUs.

==> 6rebuttal.tex <==
\newpage
\clearpage

\section{Response to Reviewer Comments}

We thank the reviewers for the time and effort they dedicated to provide valuable feedbacks on our paper. We arrange our response as follows. We first highlight the major improvements and new experiment results. Then, we respond to each comment in detail.

\subsection{Highlights in Revised Paper}
\label{sec:highlight}

The highlights in the revised paper are
\begin{itemize}
    \item \textbf{Background and Motivation} In the updated Section \ref{sec:intro}, we have added the definition of Continuous Time Dynamic Graphs (CTDGs) and Discrete Time Dynamic Graphs (DTDGs) and explained why we aim at supporting the more general CTDGs in TGL. We have also explained why it is hard to implement TGNNs on existing graph frameworks and why we need a new framework for TGNNs.
    \item \textbf{Parallel Temporal Sampler} In the updated Section \ref{sec:tglsampler}, we have added a formal definition of the proposed T-CSR data structure as well as how the T-CSR data structure is maintained during the sampling process. We have also re-structured the Section into three parts with the T-CSR data structure, sampling, and parallel sampling. We have also clarified how our T-CSR data structure can be used to insert and delete events of nodes and edges.
    \item \textbf{Random Chunk Scheduling Technique} In the updated Section \ref{sec:tglngpu}, we have replaced the Figure that was depicting the proposed random chunk scheduling technique with Algorithm \ref{alg:shce} to enhance clarity on the developed technique. We have also added a more detailed description on the proposed technique.
    \item \textbf{Experiments} In the updated Section \ref{sec:expsample}, we have added more details on the implementation of the baseline samplers and on the speedup provided by our parallel temporal sampler. For completion, in the updated Section \ref{sec:expsmall} we also have included the results of two public small-scale datasets -- the LastFM and MOOC datasets. We have also depicted the runtime of each individual step in the updated Figure \ref{fig:wiki}.
\end{itemize}

\subsection{Response to Meta-Reviewer}

\begin{enumerate}[1.]
    \item \textbf{Improve the technical exposition on the system design decisions and make the description of the techniques more rigorous and self-contained.}\\
    In the revised paper, we have added further details on the system design of TGL, especially the parallel temporal sampler and the random chunk scheduling technique. For more details, please refer to our responses to \textbf{\underline{R1.W1}}, \textbf{\underline{R1.W2/D2}}, \textbf{\underline{R2.D1}}, \textbf{\underline{R3.D1}}, and \textbf{\underline{R3.D3/D4/D5/D7}}.
    \item \textbf{Provide the missing details and further explanations of the empirical results. Provide more qualitative and quantitative justification of temporal GNN vs regular prior GNN methods/tools.}\\
    In the updated Section \ref{sec:expsample}, we have added more details on the baseline samplers and explained the speedup achieved by TGL. Please refer to our response to \textbf{\underline{R2.D1/D2}} for more details. In the updated Figure \ref{fig:wiki}, we have included the detailed execution time of each component in TGL. Please refer to our response to \textbf{\underline{R2.D3}} for more details. In the updated Section \ref{sec:expsmall}, we have justified the accuracy improvements of TGL compared with each baselines. Please refer to our response to \textbf{\underline{R3.D1}} for more details.
    \item \textbf{Add another standard public dataset from the literature for the experiments, e.g., LastFM song listens.}\\
    In the updated Section \ref{sec:expsmall}, we have added the results on two public datasets. Please refer to our response to \textbf{\underline{R3.D2}} for more details.
\end{enumerate}

\subsection{Response to Reviewer \#1}
\begin{enumerate}[1.]
    \item \textbf{\underline{W1}: The challenging for temporal GNN is not well justified, given several public GNN framework (DGL and PyG) are available.}\\
          In the updated Section \ref{sec:intro}, we have justified the motivation to develop a unified framework for TGNN. These general GNN frameworks (DGL and PyG) are mainly designed for static graphs where their data structures are not designed to efficiently store and access the dynamic graphs. In addition, they do not provide important modules in TGNNs like temporal neighbor samplers, node memory, and message passing schemes on multiple snapshots. The users need to write at least hundreds of lines of code to compose a TGNN model using DGL or PyG. By contrast, TGL users can simply to write configuration files to compose various TGNN models. The lack of a TGNN framework could also be reflected by the fact that recent TGNN works like TGAT and TGN still purely rely on basic machine learning frameworks Tensorflow and PyTorch in their experiments.
    \item \textbf{\underline{D1}: As we know CSR is very difficult for dynamic updates, since all edges are stored in the consecutive array. I do not understand how the proposed temporal CSR handle the edge or node updates, including insertion and deletions. It seems that the temporal graph in in this paper refer to a graph with temporal information on edges; but they are still static.}\\
          In the updated Section \ref{sec:intro} and Section \ref{sec:tglsampler}, we have added the clarification that the proposed T-CSR data structure is designed to support efficient offline TGNN training. In the offline training setup, the entire training (dynamic) graph is known in advance. Hence, we can allocate exact space for all the nodes and edges in the training graphs before training. We have also added a note on handling inserting, updating, and deleting events on the proposed T-CSR data structure. For the dynamic graphs that contain updating and deleting events, we follow TGN \cite{tgn} to treat each updating or deleting event independently and generate a standalone mail for each such event. However, we have also added the clarification that the T-CSR data structure could also supports dynamic graphs with the inserting and deleting events. We can treat the inserting and deleting events as standalone node or edges events with an additional validation array with size $|E|$ that marks whether an edge is valid or not. This validation array needs to be updated after finishing one mini-batch. During sampling, the invalid edges could be simply ignored.\\
          To address the online training or inference setting where the dynamic graph is streamed in, the T-CSR data structure could be modified to a List of List (LIL) or List of Array (LIA) data structure where the insert operation is cheaper than CSR. Our future work attempts to address this issue by implementing such data structure and designing hardware accelerator for online sampling.
    \item \textbf{\underline{W2/D2}: Author should provide more system implementation details of TGL.}\\
          In the revised paper, we have provide more details on the implementation details of TGL. Please refer to the \textbf{Parallel Temporal Sampler} and \textbf{Random Chunk Scheduling Technique} items in Section \ref{sec:highlight}.
\end{enumerate}

\subsection{Response to Reviewer \#2}
\begin{enumerate}[1.]
    \item \textbf{\underline{D1}: Authors claim the speedup of TGL's sampler compared with the baselines' samplers in the paper. Though it is proven with the experimental results, more details about the baselines' samplers need to be provided, as well as the details for the reason of the time improvement.}\\
          In the updated Section \ref{sec:expsample}, we have added description of the baseline samplers in the open-sourced code and the reasons of the time improvement. The main factors for the time improvements are
          \begin{enumerate}
              \item The proposed T-CSR data structure reduce the time complexity of identifying the candidate neighbors to sample from in one epoch from $\mathcal{O}(|E|\log|E|)$ to $\mathcal{O}(|E|)$. TGAT has lower speedup numbers than TGN because TGAT uses the timestamps of the neighbors to sample multi-hop neighbors. Please refer to Section \ref{sec:tglsampler} for more details. In addition, the T-CSR data structure uses contiguous memory to store the entire graph structure, which potentially leads to better cache performance.
              \item Our parallel temporal sampler exploits data parallelism by adding element-wise lock to avoid the race condition in the pointer arrays, which greatly reduces the time spent in selecting the neighbors (Figure \ref{fig:samp}.b).
              \item Our parallel temporal sampler is implemented in C++ and integrated to the main Python training program using PyBind11 where the baseline samplers are directly implemented in Python. C++ is more efficient than Python in such CPU heavy workloads.
          \end{enumerate}
    \item \textbf{\underline{D2}: In Table 4. (1) why the improvement ratio for DySAT is not included? (2) For TGN, the time for 8 threads is 0.46s but 0.039s with 32 threads. I think it is a typo here.}\\
          (1) We pick DySAT as a representative sampling method for snapshot-based TGNNs. However, there is no baseline available for DySAT sampler since DySAT adopts full neighbor training strategy.\\
          (2) Yes, it is a typo and we have corrected it.
    \item \textbf{\underline{D3}: Since there are five components in the framework TGL. I think the performance of different `mailbox' and `memory updater' can also be evaluated and included in the paper.}\\
          In the updated Figure \ref{fig:wiki}, we have further broke down the execution times to the six individual steps as shown in Figure \ref{fig:tgnn}. We have also added a clarification of the runtime breakdown in Section \ref{sec:expsmall}. In PyTorch, the GPU kernels are executed in asynchronous mode in order to overlap the operations on CPU and GPU. Measuring the time in each individual step requires the GPU kernels to be executed in synchronous mode, which leads to around 15\% overhead in the execution time compared with the default asynchronous execution. The overhead primarily comes from the data copying from CPU to GPU (step \textcircled{\small 3}) and the sampling and indexing (step \textcircled{\small 1} and \textcircled{\small 2}) which could either be overlapped with itself or with operations in the previous mini-batch. However, we believe the updated time breakdown provides more information on the runtime of each module in TGL.
    \item \textbf{\underline{D4}: There is a 404 error with the link provided by the authors. This paper proposed a framework for temporal neural networks and two large-scale temporal graphs. These can be important for the researchers. The authors are suggested to make the related code and data available as soon as possible to increase the impact of this work.}\\
          There is an internal process in AWS before the code and data can be made public available. We are working on it and will release the code and data as soon as possible.
\end{enumerate}

\subsection{Response to Reviewer \#3}
\begin{enumerate}[1.]
    \item \textbf{\underline{D1}: The experiments did not give much insights into how could the accuracies of the TGNN methods be kept or even improved after TGL techniques are used.}\\
          In the updated Section \ref{sec:expsmall}, we have explained the improvement in accuracy of TGL. From the algorithm perspective, TGL applies batch normalization in-between each layer, which increases the accuracy on JODIE and TGAT. Beside the added batch normalization on TGAT and JODIE, the other neural network architectures and training algorithms implemented in TGL are exactly the same as the baseline TGNNs. Due to the fast training speed of TGL, we are able to explore more hyper-parameters and achieve higher accuracy on TGN and TGAT due to better convergence. When training with large batch size, we have shown the effectiveness of our random chunk scheduling technique in Section \ref{sec:exprand}.
    \item \textbf{\underline{D2}: There are many data sets used in the literature (such as Last FM song listens). Why are only two datasets considered? The proposed techniques are purely empirical. Testing TGL on more datasets is necessary to investigate the behaviors (such as robustness) of TGL. If page limitation is an issue, such results can be placed in a technical report.}\\
          In the updated Section \ref{sec:expsmall}, we have included the results on two additional public datasets -- the LastFM and MOOC datasets. The LastFM datasets is a user-song dataset from the popular music website last.fm while the MOOC datasets is a user-activity dataset from the MOOC social network. However, since all baseline code except JODIE \cite{jodie} is not evaluated on these two datasets and does not support feature-less graphs, we believe there is no substantial value in comparing the performance of TGL with the baseline code on these two datasets. In the updated Section \ref{sec:intro} and Section \ref{sec:expds}, we have justified our choice of the two small-scale datasets Wikipedia and Reddit as well as the motivation to look for larger datasets.\\
          We choose the Wikipedia and Reddit datasets for the following reasons: (1) they both have an authentic 172-dimensional edge features while other datasets typically do not have edge features and have to use random features in the experiments, and (2) the state-of-the-art TGNN works (TGAT \cite{tgat}, TGN \cite{tgn}, APAN \cite{apan}) are optimized and evaluated on these two datasets, which provides comprehensive and fair baselines.\\
          On the other hand, these existing datasets only have few thousands of nodes and few millions of edges. Worse still, they are all bipartite graphs with only a few binary node labels. We believe these small-scale datasets do not reflect real-world production-scale dynamic graphs and are not capable of benchmarking various TGNN variants. Hence, we pre-process two large-scale datasets -- the GDELT and MAG datasets with 0.2 billion and 1.3 billion edges. These large-scale datasets come with node and/or edge features and have more 42 million and 1.4 million node labels for the dynamic node classification task. We will also publish these two large-scale datasets to benefit future researches.
    \item \textbf{\underline{D3}: The proposed T-CSR data structure is not formally defined. It is only illustrated in Figure 3 and described casually.}\\
          In the updated Section \ref{sec:tglsampler}, we have added more details of the proposed T-CSR data structure, including a formal definition and the space complexity analysis. We have also re-organize the Section and added three sub-titles -- the T-CSR data structure, sampling, and parallel sampling to provide a clearer description of the proposed parallel temporal sampler. We have also added a note on the handling of inserting, updating, and deleting events. Please refer to our response to \textbf{\underline{R2.D2}} for more details.
    \item \textbf{\underline{D4}: In Algorithm 1, the technical jargon DGL MFG is not even elaborated.}\\
          In the updated Section \ref{sec:tglsampler}, we have added description about DGL Message Flow Graph (MFG). The DGL MFG is a data structure used by DGL which contains information needed in the forward and backward propagation in a graph block of one mini-batch.
    \item \textbf{\underline{D5/6}: The random chunk scheduling technique is only briefly sketched. The technique is not formally defined. Figure 4 is not understandable. Its caption contains much technical jargon.}\\
          To better explain the proposed random chunk scheduling technique, in the updated Section \ref{sec:tglngpu}, we have removed Figure 4 and added a detailed algorithm Algorithm \ref{alg:shce} describing how the random chunk scheduling technique is applied in the training process. We have also revised the Section with a new title that better summarizes the motivation of our random chunk scheduling technique. In the updated section, we first state that training with large batch sizes leads to less learned inter-batch dependencies in each epoch. Then, we point out that our random chunk scheduling technique allows the TGNN models to learn different inter-batch dependencies in different epochs. With enough number of training epochs and small chunk size, the TGNN models trained with random chunk scheduling technique and large batch size can learn the same amount of inter-batch dependencies as the TGNN models train with small batch size. Lastly, we sketched the multi-GPU training strategy, where more details are provided in Section \ref{sec:explarge}.
    \item \textbf{\underline{D7}: Typos.}\\
          We have corrected these typos. For the snapshot durations, the numbers are for the snapshot duration of each dataset. In each dataset, the durations of the consecutive snapshots are constant. We have rewritten this sentence to eliminate the disambiguation. 
\end{enumerate}
